Make Sure You're Unsure: A Framework for Verifying Probabilistic Specifications

Most real world applications require dealing with stochasticity like sensor noise or predictive uncertainty, where formal specifications of desired behavior are inherently probabilistic. Despite the promise of formal verification in ensuring the reliability of neural networks, progress in the direction of probabilistic specifications has been limited. In this direction, we first introduce a general formulation of probabilistic specifications for neural networks, which captures both probabilistic networks (e.g., Bayesian neural networks, MC-Dropout networks) and uncertain inputs (distributions over inputs arising from sensor noise or other perturbations). We then propose a general technique to verify such specifications by generalizing the notion of Lagrangian duality, replacing standard Lagrangian multipliers with "functional multipliers" that can be arbitrary functions of the activations at a given layer. We show that an optimal choice of functional multipliers leads to exact verification (i.e., sound and complete verification), and for specific forms of multipliers, we develop tractable practical verification algorithms. We empirically validate our algorithms by applying them to Bayesian Neural Networks (BNNs) and MC Dropout Networks, and certifying properties such as adversarial robustness and robust detection of out-of-distribution (OOD) data. On these tasks we are able to provide significantly stronger guarantees when compared to prior work -- for instance, for a VGG-64 MC-Dropout CNN trained on CIFAR-10, we improve the certified AUC (a verified lower bound on the true AUC) for robust OOD detection (on CIFAR-100) from $0\% \rightarrow 29\%$. Similarly, for a BNN trained on MNIST, we improve on the robust accuracy from $60.2\% \rightarrow 74.6\%$. Further, on a novel specification -- distributionally robust OOD detection -- we improve the certified AUC from $5\% \rightarrow 23\%$.

==> backup.tex <==
\section{Probabilistic Specifications}\label{sec:specs}
First, we introduce the relevant notation.
Next, we provide examples for several desirable probabilistic specifications, and then introduce a general problem formulation 
that captures these specifications. 

\subsection{Notation}
We consider networks $\phi$ composed of a sequence of possibly stochastic layers $\pi_1, \ldots \pi_K$, where $\pi_k\br{x_{k}|x_{k-1}}$ denotes the probability that the output of layer $k$ is $x_k$ when its input is $x_{k-1}$. 
We write $x_{k} \sim \pi_k\br{x_{k-1}}$ to denote that $x_k$ is sampled from the distribution over outputs of layer $k$ given input $x_{k-1}$ to layer $k$.
We assume that the layers $\pi_k\br{x}$ have the form $\sigma(\tilde{w}x+\tilde{b})$, where $\sigma$ is a non-linear activation function (e.g., $\relu$, sigmoid, $\texttt{MaxOut}$), $\tilde{w}$ and $\tilde{b}$ are random variables. 
The stochasticity for layer $\pi_k$  is assumed to be statistically independent of the stochasticity at other layers.
For a BNN, $\tilde{w}$ and $\tilde{b}$ follow a diagonal Gaussian distribution, and for a MC-Dropout network they follow a Bernoulli-like distribution. 




Let $p_0$ denote a distribution over the inputs $\X$. We assume that set of outputs $\Y$ is a subset of $\R^l$ (unless specified otherwise), where $l$ is the number of labels, and the output of the NN are logits corresponding to unnormalized log-confidence scores assigned to the labels $\{1, \ldots, l\}$.  
Note that the output from the neural network $\phi: \Pcal\br{\X} \to \Pcal\br{\Y}$ for a given $p_0$ is a distribution over $\Y$, we denote this distribution by $p_y$. 
For a single input $x \in \mathcal{X}$, we abuse notation, and write $\phi(x)$ 
to denote the NN output from acting on $x$.


\subsection{Examples of Specifications}\label{sec:example_specifications}
\label{sec:probabexamples}
\paragraph{Distributionally Robust OOD Detection for Stochastic Neural Networks.} 
Here, we consider the problem of verifying that a stochastic neural network assigns low confidence scores to all labels for inputs that are OOD. 
A more general specification is one
where we want to ensure low confidence predictions (in average) on an entire sets of distributions of OOD images. 
For given distributional noise ($p_\omega$) perturbing the given OOD image ($x_\mathrm{ood}$) ,
we require that the expected softmax, defined as $\ExP{\frac{\exp\br{y_i}}{\sum_j \exp\br{y_j}}}{y \sim p_y}$, is smaller than a specified maximum confidence threshold $p_{\max}$ (for each $i$).
For a given class of 
noise distributions ($\mathcal{P}_{noise}$), 
the general verification problem is to guarantee that 
for every $p_0$ in $\mathcal{P}_0 = \{\xood + \omega: \omega \in \mathcal{P}_{noise}\}$, the 
expected softmax is below $p_{\max}$.
Robust OOD detection under bounded $\ell_\infty$ perturbations as considered in \cite{bitterwolf2020provable}
is a special case of the general problem where $\mathcal{P}_{noise}$ is a set of $\delta$ distributions over points with bounded $\ell_\infty$ norm.

\paragraph{Classification Robustness Under Perturbations.} The extension of the commonly studied robust classification problem \citep{madry2017towards}, under norm-bounded  perturbations, to the setting of probabilistic neural networks (e.g., BNNs) is another relevant probabilistic specification. 
With $\mathcal{P}_0$ defined as a set of $\delta$ input distributions centered at points within an $\epsilon$ ball of a nominal point $\xnom$, with label $i \in \{1, \ldots, l\}$: $\mathcal{P}_0 = \{\delta_x: \norm{x-\xnom} \leq \epsilon\}$, 
we wish to guarantee for every $p_0 \in \mathcal{P}_0$ that the 
stochastic NN (e.g., BNN) correctly classifies the input (in expectation).
In other words, for every $p_0 \in \mathcal{P}_0$ and for each $j$, 
we want the NN to satisfy $\ExP{\frac{\exp\br{y_i} - \exp\br{y_j}}{\sum_k \exp\br{y_k}}}{y \sim p_y} \leq 0$, i.e., the expected difference between the softmax probabilities assigned to the labels $j$ and $i$ is smaller than $0$. 

\subsection{Problem Formulation.}
We now introduce a general problem formulation that captures 
all the specifications discussed above. 
\begin{definition}[Probabilistic verification problem]
Given a (possibly stochastic) neural network $\phi: \X \to \Pcal\br{\Y}$, a set of distributions over the input $\mathcal{P}_0$ and a functional $\spec: \mathcal{P}\br{\Y} \mapsto \R$, the probabilistic verification problem is to check that the following is true:
\begin{align}
\forall \: p_0 \in \mathcal{P}_0, \: \spec\br{\phi\br{p_0}} \leq 0.\label{eq:spec}
\end{align}
\end{definition}
 We consider the following optimization version:
\begin{align}
    \texttt{OPT} = \max_{p_0 \in \mathcal{P}_0} \spec\br{\phi\br{p_0}}, \label{eq:specopt}
\end{align}
Having $\texttt{OPT} \leq 0$  here is equivalent to satisfying specification~(\ref{eq:spec}) .
In Appendix \ref{supp:specform}, we outline how this general problem formulation captures the specifications from Section \ref{sec:example_specifications}, and also 
provide further examples of relevant probabilistic specifications.

==> space_hacking.tex <==
\usepackage{enumitem}

\usepackage[small,compact]{titlesec}
\titlespacing*{\section}{0pt}{0pt plus 0pt minus 0pt}{-2pt plus 0pt minus 2pt}
\titlespacing*{\subsection}{0pt}{0pt plus 0pt minus 0pt}{0pt plus 0pt minus 0pt}
\titlespacing*{\paragraph}{0pt}{0pt plus 0pt minus 0pt}{2pt plus 0pt minus 0pt}





